Non-parametric Differentially Private Confidence Intervals for the Median

Differential privacy is a restriction on data processing algorithms that provides strong confidentiality guarantees for individual records in the data. However, research on proper statistical inference, that is, research on properly quantifying the uncertainty of the (noisy) sample estimate regarding the true value in the population, is currently still limited. This paper proposes and evaluates several strategies to compute valid differentially private confidence intervals for the median. Instead of computing a differentially private point estimate and deriving its uncertainty, we directly estimate the interval bounds and discuss why this approach is superior if ensuring privacy is important. We also illustrate that addressing both sources of uncertainty--the error from sampling and the error from protecting the output--simultaneously should be preferred over simpler approaches that incorporate the uncertainty in a sequential fashion. We evaluate the performance of the different algorithms under various parameter settings in extensive simulation studies and demonstrate how the findings could be applied in practical settings using data from the 1940 Decennial Census.

==> smooth-sens.tex <==
\subsection{Smooth Sensitivity}
\begin{definition}[$\beta$-Smooth Bounds]
For $\beta > 0$, a function $S:D^n \rightarrow \mathbb{R}^+$ is a $\beta$-smooth upper bound on the local sensitivity of $f$ if it satisfies the following:
$$ \forall x \in D^n, S(x) \ge LS_f(x); $$
$$ \forall \text{ neighboring } x,y \in D^n, S(x) \le e^\beta S(y).$$
\end{definition}

\begin{definition}[Smooth Sensitivity]
For $\beta > 0$, the $\beta$-smooth sensitivity of $f$ is
$$ S^*_{f,\beta} (x) = \max_{y \in D^n} \left( \ls(y) e^{-\beta d(x,y)} \right).$$
\end{definition}

\begin{lemma}
$\sfb$ is a $\beta$-smooth upper bound on $\ls$. In addition, $\sfb \le S(x) \forall x \in D^n$ for every $\beta$-smooth upper bound $S$ on $\ls$. 
\end{lemma}

\begin{lemma}
WLOG assume that the points in $x$ are sorted in nondecreasing order.
The smooth sensitivity of the median is 
$$ \smed(x) = \max_{k=0,\ldots,n} \left( e^{-k\beta} \max_{t=0,\ldots, k+1}(x_{m+t} - x_{m_t-k-1}) \right).$$
\end{lemma}

\begin{proof}
Let R be the range of the data. Then the global sensitivity of the median is R. Note that the local sensitivity of the median for a dataset is the maximum of the distances between the median and the points to either side of the median. I.e., for $m = (n+1)/2$, 
$$ \lsmed = \max(x_m - x_{m-1}, x_m + x_{m+1}).$$

WLOG assume that the data is centered between 0 and R. Then, by shifting $k$ points to the right or left of the median to R or 0 respectively, the median of database $x$ can be shifted anywhere in $[x_{m-k}, x_{m+k}]$. So, to maximize the local sensitivity of a database $y$ a distance $k$ away from $x$, find the widest spacing between any 2 points about the median in $x$ which are $k+1$ points apart. (Note that this is $k+1$ not $k$ since this is the local sensitivity of $y$ which is already $k$ away from $x$). I.e.,

$$ A^{(k)}(x) = \max_{y:d(x,y)=k} \lsmed(y) = \max_{0 \le i \le k+1} (x_{m + i} - x_{m+i-k-1}).$$ 

Then,

$$ \smed (x) = \max_k e^{-\beta (k} A^{(k)}(x). $$
\end{proof}


\begin{theorem}[DKW inequality]
Let $X_1, \ldots, X_n$ be real-valued i.i.d. random variables with cumulative distribution function $F(\cdot)$ and empirical distribution function $\hat{F}_n$. Then, $\forall \gamma > 0$, 

$$ P\left(\sup_{c \in \mathbb{R}} \left\vert \hat{F}_n(c) - F(c) \right\vert > \gamma\right) \le 2e^{-2n\gamma^2}.$$
\end{theorem}

\begin{lemma}
Let $X_1, \cdots, X_n$ real-valued i.i.d. random variables with cumulative distribution function $F(\cdot)$. Then for any $\gamma>0$, with probability $1-2e^{-2n\gamma^2}$,

$$ e^{-\beta n2\gamma} \le \frac{\text{SS}_\beta}{\sup_{a \le \median \le b} (b-a) e^{-\beta n (F(b)-F(a) -\frac{1}{n})} e^ {-\beta n2\gamma}} \le e^{\beta n2\gamma}.$$
\end{lemma}

\begin{proof}

Let $a = x_i$ and $b = x_j$. Then, 
\begin{align*}
 \smed (x) &= \max_{k=0,\ldots,n} \left( e^{-k\beta} \max_{t=0,\ldots, k+1}(x_{m+t} - x_{m_t-k-1}) \right) \\
	&\le \sup_{i \le n/2 \le j} (x_j - x_i) e^{- \beta (j-i-1)} \textcolor{magenta}{\text{This should be an equality right?}}\\
	&= \sup_{a \le \median \le b} (b-a) e^{-\beta n [\hat{F}_n(b) - \hat{F}_n(a) - \frac{1}{n}]}
\end{align*}

Where $\hat{F}_n$ indicates the empirical cumulative distribution function on x. The equivalence then holds since 
$$\hat{F}_n(a) = \frac{1}{n} \sum_{i=1}^n \mathbbm{1}_{x_i \le a} = \frac{i}{n}.$$
\textcolor{magenta}{There is some subtlety here when the distribution is discrete, no?}
We'd like to be able to get a bound on the smooth sensitivity given the true cumulative distribution function rather than the empirical distribution function. From the DKW inequality,

\begin{align*}
& P \left( \sup_{c \in \mathbb{R}} \left\vert \hat{F}_n(c) - F(c)  \right\vert \le \gamma \right) \ge 1 - 2e^{-2n\gamma^2}, \\
\Longleftrightarrow &P \left( \left\vert \hat{F}_n(b) - F(b) \right\vert \le \gamma \text{ and } \left\vert \hat{F}_n(a) - F(a) \right\vert \le \gamma \right) \ge 1 - 2e^{-2n\gamma^2}, \\
\Longleftrightarrow & P \left( \left\vert \left((\hat{F}_n(b) - F(b)\right) - \left(\hat{F}_n(a) - F(a)\right) \right\vert \le2\gamma \right) \ge 1 - 2e^{-2n\gamma^2}. 
\end{align*}

Then, \textcolor{magenta}{with probability $1-2e^{-2n\gamma^2}$}, we can bound $\smed$ on either side:
\begin{align*}
 \text{SS}_{\beta} =  \sup_{a \le \median \le b} (b-a) e^{-\beta n [\hat{F}_n(b) - \hat{F}_n(a) - \frac{1}{n}]} \in &\bigg[ \sup_{a \le \median \le b} (b-a) e^{-\beta n [F(b) - F(a) + 2\gamma - \frac{1}{n}]} , \\\
 	& \sup_{a \le \median \le b} (b-a) e^{-\beta n [F_n(b) - F_n(a) - 2\gamma - \frac{1}{n}]} \bigg],
\end{align*}

so

$$ e^{-\beta n2\gamma} \le \frac{\text{SS}_\beta}{\sup_{a \le \median \le b} (b-a) e^{-\beta n (F(b)-F(a) -\frac{1}{n}} e^ {-\beta n2\gamma}} \le e^{\beta n2\gamma}.$$ \textcolor{magenta}{there shouldn't be a $e^{-\beta n2\gamma}$ in the denominator right?}
\end{proof}

\begin{corollary}
There exists a distribution such that given $n$ samples, with probability $\ge \alpha$, \[\smed\ge e^{\beta-\beta\sqrt{2n\ln\left(\frac{2}{\alpha}\right)}}.\]
\end{corollary}

\begin{proof}
Let $F$ be the cumulative distribution of the function that uniform on $\{0,1\}$. Let $\gamma=\sqrt{\frac{\ln\left(\frac{2}{\alpha}\right)}{2n}}$, $a=0$ and $b=1$.
\end{proof}
